GRAML: Goal Recognition As Metric Learning

Goal Recognition (GR) is the problem of recognizing an agent's objectives based on observed actions. Recent data-driven approaches for GR alleviate the need for costly, manually crafted domain models. However, these approaches can only reason about a pre-defined set of goals, and time-consuming training is needed for new emerging goals. To keep this model-learning automated while enabling quick adaptation to new goals, this paper introduces GRAML: Goal Recognition As Metric Learning. GRAML uses a Siamese network to treat GR as a deep metric learning task, employing an RNN that learns a metric over an embedding space, where the embeddings for observation traces leading to different goals are distant, and embeddings of traces leading to the same goals are close. This metric is especially useful when adapting to new goals, even if given just one example observation trace per goal. Evaluated on a versatile set of environments, GRAML shows speed, flexibility, and runtime improvements over the state-of-the-art GR while maintaining accurate recognition.

==> time.tex <==
\begin{table}[]
\scriptsize
\caption{Runtime (reported in seconds) of the different algorithms averaged over 400 instances with varying configurations.  GRAQL is evaluated on Minigrid, and GRDRL is evaluated on the others. TO means that the algorithm times out after 2 hours.} %\matan{I suggest writing how many hours rather than TO because all G is TO for GRAQL}}
\label{tab:runtime}
\begin{tabular}{|c|rr|rr|rr|rr|}
\hline
\multicolumn{1}{|l|}{}                                  & \multicolumn{2}{c|}{Minigrid}                            & \multicolumn{2}{c|}{PointMaze}                           & \multicolumn{2}{c|}{Parking}                             & \multicolumn{2}{c|}{Panda}                                \\ \hline
Phase                                                   & \multicolumn{1}{c|}{G}          & \multicolumn{1}{c|}{I} & \multicolumn{1}{c|}{G}          & \multicolumn{1}{c|}{I} & \multicolumn{1}{c|}{G}          & \multicolumn{1}{c|}{I} & \multicolumn{1}{c|}{G}           & \multicolumn{1}{c|}{I} \\ \hline
\begin{tabular}[c]{@{}c@{}}GRAQL /\\ GRDRL\end{tabular} & \multicolumn{1}{r|}{TO}         & 0.04                   & \multicolumn{1}{r|}{TO}         & 2.56                   & \multicolumn{1}{r|}{TO}         & 2.49                   & \multicolumn{1}{r|}{TO}          & \textbf{2.24}          \\ \hline
BG-GRAML                                                & \multicolumn{1}{r|}{\textbf{0}} & \textbf{0.03}          & \multicolumn{1}{r|}{\textbf{0}} & \textbf{1.47}          & \multicolumn{1}{r|}{\textbf{0}} & 2.17                   & \multicolumn{1}{r|}{}            &                        \\ \hline
GC-GRAML                                                & \multicolumn{1}{r|}{}           &                        & \multicolumn{1}{r|}{}           &                        & \multicolumn{1}{r|}{36}         & \textbf{1.54}          & \multicolumn{1}{r|}{\textbf{87}} & 5.29                   \\ \hline
\end{tabular}
\end{table}
